Speech Translation with Large Language Models: An Industrial Practice

Given the great success of large language models (LLMs) across various tasks, in this paper, we introduce LLM-ST, a novel and effective speech translation model constructed upon a pre-trained LLM. By integrating the large language model (LLM) with a speech encoder and employing multi-task instruction tuning, LLM-ST can produce accurate timestamped transcriptions and translations, even from long audio inputs. Furthermore, our findings indicate that the implementation of Chain-of-Thought (CoT) prompting can yield advantages in the context of LLM-ST. Through rigorous experimentation on English and Chinese datasets, we showcase the exceptional performance of LLM-ST, establishing a new benchmark in the field of speech translation. Demo: https://speechtranslation.github.io/llm-st/.

==> Sections/040related.tex <==
\textbf{ASR}~


\textbf{ST}~

==> Tables/hours_zhen.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|cccc}
        Models & Languages & Total hours of speech & Hours of Zh ASR & Hours of Zh-En \\
        SeamlessM4T & Multilingual & 470k & 9k & 18k \\
        Whisper & Multilingual& 680k & 23k & 11k \\
        AudioPaLM-2 & Multilingual & 18k & 120 & 10 \\
        \method & Bilingual & 52k & 15k & 11k 
    \end{tabular}
    \caption{Caption}
    \label{tab:hours_zhen}
\end{table}

==> Tables/main_enzh.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{3.0pt}
    \begin{tabular}{l|cccccc}
        \toprule
        & \multicolumn{2}{c}{Public} & \multicolumn{3}{c}{In-house} & \multirow{2}{*}{Avg}\\
        \cmidrule{2-3} \cmidrule{4-6}
        Models & GigaST & MuSTC-v2 & News & Talk & Video  &    \\
        \midrule
        \textit{End-to-end Models} \\
        SeamlessM4T & 26.4 / 49.9 / 78.0 &	21.1 / 53.4 / 79.6 & 26.4 / 56.5 / 82.3 & 25.0 / 54.6 / 81.0 & 23.0 / 47.6 / 75.1 & 24.3 / 52.4 / 79.2\\ 
        Encoder-Decoder & 40.5 / 60.0 / 83.9 & 27.3 / 60.8 / 84.1 & 36.8 / 64.4 / 86.4 & 30.3 / 63.8 / 80.2 & 36.2 / 62.0 / 77.6 & 34.2 / 62.4 / 82.4 \\
        \midrule
        \textit{Cascaded Systems} \\
        Whisper + MT-G & 38.8 / 60.9 / 84.2 & 26.7 / 61.1 / 83.7 & 36.1 / 64.6 / 86.0 & 33.9 / 64.7 / 86.1 & 35.6 / 65.6 / 84.8 & 34.2 / 63.4/ 85.0\\
        Whisper + MT-B & 40.9 / 61.4 / 84.3 & 28.2 / 61.4 / 83.8 & 37.1 / 65.2 / 86.2 & 34.7 / 64.0 / 85.7 & 38.7 / 64.5 / 84.4 & 35.9 / 63.3 /84.9\\
        Whisper + GPT3.5 & 32.7 / 61.9 / 84.8 & 25.2 / 62.2 / 84.6  & 32.3 / 65.7 / 86.6 & 31.4 / 65.1 / 86.5 & 32.7 / 64.9 / 84.6 & 30.9 / 64.0 / 85.4\\
        ST product B & 40.9 / 58.6 / 82.4 &	28.2 / 60.6 / 83.6 & 36.4 / 62.3 / 84.2 & 31.1 / 62.5 / 84.6 & 	37.5 / 62.7 / 84.1 & 34.8 / 61.3 / 83.8 \\
        \midrule
        \method & 39.6 / 62.8 / 85.3 & 29.6 / 63.5 / 86.0 &	36.6 / 66.3 / 87.2 & 36.2 / 65.5 / 86.8 & 39.8 / 65.8 / 85.7 & 36.4 / 64.8 / 86.2 \\
        \quad -COT \\
        \quad ASR + MT \\
        \bottomrule
    \end{tabular}
    \caption{BLEU, BLEURT and COMET score of different systems for En-Zh translation}
    \label{tab:st_enzh}
\end{table}


==> Tables/main_st_zhen_bc_hours.tex <==
% \begin{table}[t]

\begin{wraptable}{r}{0.5\linewidth}
    \centering
    \footnotesize
    \setlength\tabcolsep{3.0pt}
    \begin{tabular}{l|rrr|cccc|c}
        \toprule
        &  &   &   & \multicolumn{1}{c}{Public} & \multicolumn{3}{c|}{In-house} & \multirow{2}{*}{Avg}\\
        \cmidrule{5-5} \cmidrule{6-8}
        Models & Speech (h) & Zh ASR (h) & Zh-En ST (h) & CoVoST2 &  News & Talk & Live  &    \\
        \midrule
        \textit{End-to-end Models} \\
        SeamlessM4T & 470k & 9k & 18k & 22.3 / 77.1  & 22.5 / 80.5 & 18.4 / 79.8 & 13.3 / 72.1 & 19.5 / 77.5 \\ 
        Whisper ST & 680k & 23k & 11k & 17.0 / 69.7 & 25.1 / 79.6 & 20.5 / 79.4 & 17.5 / 72.6 & 20.0 / 75.3\\
        SpeechLLaMA & - & - & -& 12.3 / -  & - & - & - & - \\
        AudioPaLM-2 (8B) & 18k & 120 & 10 & 25.5 / - & - & - & - & - \\
        mSLAM-CTC (2B) & - & - & - & 10.0 / - & - & - & - & - \\
        \midrule
        \textit{Cascaded Systems} \\
        Whisper + Google Trans & - & - & - & 26.7 / 79.2  &  42.1 / 86.1 & 24.4 / 83.7 & 25.3 / 78.6 & 29.6 / 81.9 \\
        % Whisper + MT-B & 26.0 / 78.6 &  43.2 / 86.0  & 23.1 / 83.1 & 25.5 / 78.4 & 29.5 / 81.5\\
        Whisper + GPT3.5 &  - & - & -  & 21.6 / 79.0 & 33.3 / 86.3 & 20.5 / 84.5 & 19.5 / 78.9 & 23.7 / 82.2 \\
        ST product B &  - & - & - & 29.9 / 80.5 & \textbf{45.9} / 86.5 & 23.2 / 82.5 & 27.7 / 80.9 & 31.7 / 82.6\\
        \midrule
        \method & 52k & 11k & 15k & \textbf{37.6} / \textbf{83.7} & 44.9 / \textbf{87.2} & \textbf{25.9} / \textbf{84.6} & \textbf{28.2} / \textbf{81.4} & \textbf{34.1} / \textbf{84.2}\\
            \quad - CoT &  - & - & - & 17.8 / 82.7 & 42.9 / 86.7 & 25.5 / 84.3  & 26.6 / 80.1 & 28.2 / 83.5\\
            \quad ASR + MT &  - & - & -  & 15.5 / 82.1 & 35.4 / 85.4 & 20.9 / 83.5  & 19.9 / 78.3 & 22.9 / 82.3 \\   
        \bottomrule
    \end{tabular}
    \caption{BLEU and COMET score of different systems for Zh-En translation}
    \label{tab:st_zhen_bc}

\end{wraptable}
% \end{table}



==> Tables/main_zhen.tex <==
\begin{table}[t]
    \centering
    \setlength\tabcolsep{3.0pt}
    \begin{tabular}{l|ccccc}
        \toprule
        & \multicolumn{1}{c}{Public} & \multicolumn{3}{c}{In-house} & \multirow{2}{*}{Avg}\\
        \cmidrule{2-2} \cmidrule{3-5}
        Models & CoVoST2 &  News & Talk & Live  &    \\
        \midrule
        \textit{End-to-end Models} \\
        SeamlessM4T & 22.3 / 55.1 / 77.1  & 22.5 / 61.6 / 80.5 & 18.4 / 61.3 / 79.8 & 13.3 / 52.3 / 72.1 & 19.5 / 57.8 / 77.5 \\ 
        Whisper ST & 17.0 / 46.3 / 69.7 & 25.1 / 60.1 / 79.6 & 20.5 / 59.0 / 79.4 & 17.5 / 50.0 / 72.6 & 20.0 / 53.9 / 75.3\\
        SpeechLLaMA & 12.3 / - / -  & - & - & - & - \\
        AudioPaLM-2 8B & 25.5 / - / - & - & - & - & - \\
        mSLAM-CTC (2B) & 10.0 / - / - & \\
        \midrule
        \textit{Cascaded Systems} \\
        Whisper + MT-G & 26.7 / 56.6 / 79.2  &  42.1 / 69.3 / 86.1 & 24.4 / 63.3 / 83.7 & 25.3 / 56.0 / 78.6 & 29.6 / 61.3 / 81.9 \\
        Whisper + MT-B & 26.0 / 56.1 / 78.6 &  43.2 / 68.9 / 86.0  & 23.1 / 62.4 / 83.1 & 25.5 / 56.1 / 78.4 & 29.5 / 60.9 / 81.5\\
        Whisper + GPT3.5 & 21.6 / 58.3 / 79.0 & 33.3 / 70.7 / 86.3 & 20.5 / 66.4 / 84.5 & 19.5 / 59.0 / 78.9 & 23.7 /	63.6 / 82.2 \\
        ST product B & 29.9 / 58.9 / 80.5 & 45.9 / 70.7 / 86.5 & 23.2 / 63.0 / 82.5 & 27.7 / 60.8 / 80.9 & 31.7 / 63.4 / 82.6\\
        \midrule
        \method & 37.6 / 64.0 / 83.7 & 44.9 / 73.4 / 87.2 & 25.9 / 66.5 / 84.6 & 28.2 / 62.1 / 81.4 & 34.1 / 66.5 / 84.2\\
            \quad -COT & 17.8 / 63.2 / 82.7 & 42.9 / 71.2 / 86.7 & 25.5 / 84.3  & 26.6 / 80.1\\
            \quad ASR + MT & 15.5 / 62.7 / 82.1 & 35.4 / 69.9 / 85.4 & 20.9 / 83.5  & 19.9 / 78.3 \\   
        \bottomrule
    \end{tabular}
    \caption{BLEU, BLEURT and COMET score of different systems for Zh-En translation}
    \label{tab:st_zhen}
\end{table}


